The Phong Surface: Efficient 3D Model Fitting using Lifted Optimization

Realtime perceptual and interaction capabilities in mixed reality require a range of 3D tracking problems to be solved at low latency on resource-constrained hardware such as head-mounted devices. Indeed, for devices such as HoloLens 2 where the CPU and GPU are left available for applications, multiple tracking subsystems are required to run on a continuous, real-time basis while sharing a single Digital Signal Processor. To solve model-fitting problems for HoloLens 2 hand tracking, where the computational budget is approximately 100 times smaller than an iPhone 7, we introduce a new surface model: the `Phong surface'. Using ideas from computer graphics, the Phong surface describes the same 3D shape as a triangulated mesh model, but with continuous surface normals which enable the use of lifting-based optimization, providing significant efficiency gains over ICP-based methods. We show that Phong surfaces retain the convergence benefits of smoother surface models, while triangle meshes do not.

==> figs/HoloLensDatasetResult/HololensPerf.tex <==
% !TEX root = ..\..\SubdivHandTracking.tex
%

\begin{minipage}[b]{\columnwidth}
	\begin{tikzpicture}
	\begin{axis}[
	xlabel={Error threshold $\epsilon$ (mm)},
	ylabel={\averagemetriclabel{\epsilon}},
	ylabel style={align=flush center,text width=\yaxiswidth,yshift=-0.1cm},
	xticklabel={\pgfmathparse{100*\tick}$\pgfmathprintnumber{\pgfmathresult}0$},
	yticklabel={\pgfmathparse{100*\tick}$\pgfmathprintnumber{\pgfmathresult}$},
	width=0.3\columnwidth,
	height=\plotheight,
	ymax=1,
	xmax=0.03,
	legend style={anchor=south,at={(1.2, 1.1)},/tikz/every even column/.append style={column sep=0.02\columnwidth}},
	legend columns=3,
	reverse legend
	]
\addplot[chira5] table[header=false] {figs/HololensDatasetResult/Data/bin_x86_SubdivDeg2_forearm_avg_err.data}; \addlegendentry{ApproxLoopDeg2}
\addplot[chira4] table[header=false] {figs/HololensDatasetResult/Data/bin_x86_SubdivDeg3_forearm_avg_err.data}; \addlegendentry{ApproxLoopDeg3}	
\addplot[chira3] table[header=false] {figs/HololensDatasetResult/Data/bin_x86_PlanarTriangles_forearm_avg_err.data}; \addlegendentry{PlanarTriangles}
\addplot[chira2] table[header=false] {figs/HololensDatasetResult/Data/bin_x86_SubdivSurface_forearm_avg_err.data}; \addlegendentry{LoopSubdiv}
\addplot[chira1] table[header=false] {figs/HololensDatasetResult/Data/bin_x86_PhongSurface_forearm_avg_err.data}; \addlegendentry{PhongSurface (This paper)}	
	
	\end{axis}
	\begin{axis}[
		xlabel={Error threshold $\epsilon$ (mm)},
		ylabel={\maxmetriclabel{\epsilon}},
		ylabel style={align=flush center,text width=\yaxiswidth,yshift=-0.1cm},
		xticklabel={\pgfmathparse{100*\tick}$\pgfmathprintnumber{\pgfmathresult}0$},
		yticklabel={\pgfmathparse{100*\tick}$\pgfmathprintnumber{\pgfmathresult}$},
		width=0.3\columnwidth,
		height=\plotheight,
		xshift=0.5\columnwidth,
		ymax=1,
		xmax=0.03
		]
	\addplot[chira5] table[header=false] {figs/HololensDatasetResult/Data/bin_x86_SubdivDeg2_forearm_max_err.data};
	\addplot[chira4] table[header=false] {figs/HololensDatasetResult/Data/bin_x86_SubdivDeg3_forearm_max_err.data};	
	\addplot[chira3] table[header=false] {figs/HololensDatasetResult/Data/bin_x86_PlanarTriangles_forearm_max_err.data};
	\addplot[chira2] table[header=false] {figs/HololensDatasetResult/Data/bin_x86_SubdivSurface_forearm_max_err.data}; 
	\addplot[chira1] table[header=false] {figs/HololensDatasetResult/Data/bin_x86_PhongSurface_forearm_max_err.data};
		\end{axis}
	\end{tikzpicture}\vskip-3pt
	\subcaption{ Average joint error (left) and max joint error (right) of tracking on the HoloLens 2 (with 45fps config) on their depth dataset.}\label{subfig:hololens-err}
\end{minipage}\\[6pt]


\begin{minipage}[b]{\columnwidth}
	\begin{tikzpicture}
	\begin{axis}[
	xlabel={\averagemetriclabel{20}mm},
	ylabel={Time (in fps)},	
	%xlabel={Number of starting points},
	ylabel style={align=flush center,text width=\yaxiswidth,yshift=-0.1cm},
	yticklabel={$\hphantom{10}\pgfmathprintnumber{\tick}$},
	legend pos=north east,
	width=0.7\columnwidth,
	height=\plotheight,
	ymin=0,
	ymax =400.0,
	xmin=50,
	xmax = 100,
	legend style={yshift=10pt}
	%		Enable error bars for standard deviation:
	%		every axis plot/.append style={
	%			error bars/y dir=both, error bars/y explicit
	%		}
	]	
	\addplot[only marks, mark options={draw=chira5,fill=chira5},]  table[header=false] {figs/HoloLensDatasetResult/Data/ApproxLoopDeg2Perf.dat}; 
	\addplot[only marks, mark options={draw=chira4,fill=chira4},]  table[header=false] {figs/HoloLensDatasetResult/Data/ApproxLoopDeg3Perf.dat}; 
	\addplot[only marks, mark options={draw=chira3,fill=chira3},]  table[header=false] {figs/HoloLensDatasetResult/Data/PlanarTrianglesPerf.dat}; 
	\addplot[only marks, mark options={draw=chira2,fill=chira2},] table[header=false] {figs/HoloLensDatasetResult/Data/ApproxLoopPerf.dat}; 	
	\addplot[only marks, mark options={draw=chira1,fill=chira1},]  table[header=false] {figs/HoloLensDatasetResult/Data/PhongSurfacePerf.dat}; 
	\end{axis}

	\end{tikzpicture}%
	\subcaption{The perf (timings on model-fitting session) v.s. accuracy (percentage of dataset with avg joint error less than 20mm) for the hand tracking on HoloLens 2 with 45fps config.}\label{subfig:hololens-perf}
\end{minipage}\vskip-3pt




==> figs/HoloLensDatasetResult/HololensPerf6DoF.tex <==
% !TEX root = ..\..\SubdivHandTracking.tex
%


\begin{minipage}[b]{\columnwidth}
	\begin{tikzpicture}
	\begin{axis}[
	xlabel={Error threshold $\epsilon$ (mm)},
	ylabel={\averagemetriclabel{\epsilon}},
	ylabel style={align=flush center,text width=\yaxiswidth,yshift=-0.1cm},
	xticklabel={\pgfmathparse{100*\tick}$\pgfmathprintnumber{\pgfmathresult}0$},
	yticklabel={\pgfmathparse{100*\tick}$\pgfmathprintnumber{\pgfmathresult}$},
	width=0.3\columnwidth,
	height=\plotheight,
	ymax=1,
	xmax=0.03,
	legend style={anchor=south,at={(1.2, 1.1)},/tikz/every even column/.append style={column sep=0.02\columnwidth}},
	legend columns=2,
	reverse legend
	]

	\addplot[chira3b, dashed] table[header=false] {figs/HololensDatasetResult/Data/bin_x86_wo6DoF_PlanarTriangles_forearm_avg_err.data}; \addlegendentry{PlanarTriangles wo/6DoF initialiation from Dnn}
	\addplot[chira3] table[header=false] {figs/HololensDatasetResult/Data/bin_x86_PlanarTriangles_forearm_avg_err.data}; \addlegendentry{PlanarTriangles }
	%\addplot[chira2] table[header=false] {figs/HololensDatasetResult/Data/bin_x86_wo6DoF_SubdivDeg4_forearm_avg_err.data}; \addlegendentry{LoopSubdiv}
	%\addplot[chira2b, dashed] table[header=false] {figs/HololensDatasetResult/Data/bin_x86_wo6DoF_SubdivDeg4_forearm_avg_err.data}; \addlegendentry{LoopSubdiv+6DoFDnn}
	\addplot[chira1b, dashed] table[header=false] {figs/HololensDatasetResult/Data/bin_x86_wo6DoF_PhongSurface_forearm_avg_err.data}; \addlegendentry{PhongSurface wo/6DoF initialiation from Dnn}
	\addplot[chira1] table[header=false] {figs/HololensDatasetResult/Data/bin_x86_PhongSurface_forearm_avg_err.data}; \addlegendentry{PhongSurface}	
	\end{axis}

	\begin{axis}[
	xlabel={Error threshold $\epsilon$ (mm)},
	ylabel={\maxmetriclabel{\epsilon}},
	ylabel style={align=flush center,text width=\yaxiswidth,yshift=-0.1cm},
	xticklabel={\pgfmathparse{100*\tick}$\pgfmathprintnumber{\pgfmathresult}0$},
	yticklabel={\pgfmathparse{100*\tick}$\pgfmathprintnumber{\pgfmathresult}$},
	width=0.3\columnwidth,
	height=\plotheight,
	xshift=0.5\columnwidth,
	ymax=1,
	xmax=0.03
	]
\addplot[chira3b, dashed] table[header=false] {figs/HololensDatasetResult/Data/bin_x86_wo6DoF_PlanarTriangles_forearm_max_err.data}; 
\addplot[chira3] table[header=false] {figs/HololensDatasetResult/Data/bin_x86_PlanarTriangles_forearm_max_err.data};
%\addplot[chira2] table[header=false] {figs/HololensDatasetResult/Data/bin_x86_wo6DoF_SubdivDeg4_forearm_max_err.data};
%\addplot[chira2b, dashed] table[header=false] {figs/HololensDatasetResult/Data/bin_x86_wo6DoF_SubdivDeg4_forearm_avg_err.data};
\addplot[chira1b, dashed] table[header=false] {figs/HololensDatasetResult/Data/bin_x86_wo6DoF_PhongSurface_forearm_max_err.data};
\addplot[chira1] table[header=false] {figs/HololensDatasetResult/Data/bin_x86_PhongSurface_forearm_max_err.data};
	\end{axis}
	\end{tikzpicture}\vskip-3pt
	\subcaption{Average joint error (left) and max joint error (right) of HoloLens hand tracking with and without 6DoF intialization from Dnn on HoloLens depth dataset.}\label{subfig:hololens-avgErr-6dof}
\end{minipage}\\[6pt]




==> figs/HoloLensDatasetResult/HololensPerfAccuracy.tex <==
% !TEX root = ..\..\SubdivHandTracking.tex
%


\begin{minipage}[b]{0.4\columnwidth}
	\begin{tikzpicture}
	\begin{axis}[
	xlabel={\% of dataset with avg. joint err. $< 20$mm},
	ylabel={Model fitting speed \\ (in fps, larger is better)},	
	%xlabel={Number of starting points},
	ylabel style={align=flush center,text width=\yaxiswidth,yshift=-0.1cm},
	yticklabel={$\hphantom{10}\pgfmathprintnumber{\tick}$},
	legend pos=north west,
	width=0.8\columnwidth,
	height=0.6\plotheight,
	ymin=0,
	ymax =400,
	xmin=40,
	xmax = 100,
	%		Enable error bars for standard deviation:
	%		every axis plot/.append style={
	%			error bars/y dir=both, error bars/y explicit
	%		}
	]	

	\addplot[only marks, mark options={draw=chira1,fill=chira1},]  table[header=false] {figs/HoloLensDatasetResult/Data/PhongSurfacePerf.dat};  \addlegendentry{Phong}
	\addplot[only marks, mark options={draw=chira2,fill=chira2},] table[header=false] {figs/HoloLensDatasetResult/Data/ApproxLoopPerf.dat};  \addlegendentry{Subdiv.}
	\addplot[only marks, mark options={draw=chira3,fill=chira3},]  table[header=false] {figs/HoloLensDatasetResult/Data/PlanarTrianglesPerf.dat}; \addlegendentry{Tri. mesh }
	%\addplot[only marks, mark options={draw=chira5,fill=chira5},]  table[header=false] {figs/HoloLensDatasetResult/Data/ApproxLoopDeg2Perf.dat}; \addlegendentry{B\'ezier deg.2 }
	%\addplot[only marks, mark options={draw=chira4,fill=chira4},]  table[header=false] {figs/HoloLensDatasetResult/Data/ApproxLoopDeg3Perf.dat}; \addlegendentry{B\'ezier deg.3}

	\end{axis}

	\end{tikzpicture}%
\end{minipage}\vskip-3pt



